Realistic Evaluation Principles for Cross-document Coreference Resolution

We point out that common evaluation practices for cross-document coreference resolution have been unrealistically permissive in their assumed settings, yielding inflated results. We propose addressing this issue via two evaluation methodology principles. First, as in other tasks, models should be evaluated on predicted mentions rather than on gold mentions. Doing this raises a subtle issue regarding singleton coreference clusters, which we address by decoupling the evaluation of mention detection from that of coreference linking. Second, we argue that models should not exploit the synthetic topic structure of the standard ECB+ dataset, forcing models to confront the lexical ambiguity challenge, as intended by the dataset creators. We demonstrate empirically the drastic impact of our more realistic evaluation principles on a competitive model, yielding a score which is 33 F1 lower compared to evaluating by prior lenient practices.

==> tables/ecb_examples.tex <==
\begin{table*}
    \fontsize{10.5}\selectfont 
    \centering
    \resizebox{1\textwidth}{!}{
    \begin{tabular}{p{8cm}||p{8cm}}\toprule
    \multicolumn{1}{c}{\textbf{Subtopic 1}} &
    \multicolumn{1}{c}{\textbf{Subtopic 2}} \\
    \toprule

    \emph{News that \textbf{\textcolor{blue}{Barack Obama}} may \textbf{\underline{\textcolor{cadmiumorange}{name}}} \textbf{\textcolor{red}{Dr. Sanjay Gupta}} of Emory University and CNN as \textbf{\textcolor{blue}{his}} Surgeon...} 
    & 
    \emph{\textbf{\textcolor{blue}{President Obama}} will \textbf{\underline{\textcolor{darkspringgreen}{name}}} \textbf{\textcolor{chamoisee}{Dr. Regina Benjamin}} as Surgeon General in a Rose Garden announcement...} \\ \\
    
    \emph{CNN's management confirmed yesterday that \textbf{\textcolor{red}{Dr. Gupta}} had been  \textbf{\underline{\textcolor{cadmiumorange}{approached}}} by the Obama team. } 
    &
    \emph{\textbf{\textcolor{blue}{Obama}} \textbf{\underline{\textcolor{darkspringgreen}{nominates}}} new surgeon general: \textbf{\textcolor{chamoisee}{genius grant fellow Dr. Benjamin. }} \textbf{\textcolor{blue}{He}} emphasizes \textbf{\textcolor{blue}{his}} \textbf{\underline{\textcolor{darkspringgreen}{decision}}}..} 
    \\
    
    \bottomrule
    \end{tabular}}
    \caption{Example of sentences of topic 34 in ECB+. The underlined words represent events, same color represents a coreference cluster.
    Different documents describe the same event using different words (e.g name, approached), while the two predicates ``name" in the two subtopics are not coreferring. 
    % The two subtopics present a challenging case of ambiguity 
    % between the two different \emph{nominations}. 
    % in which the models need to distinguish between two different \emph{nominations}. 
    % between ``\emph{name} Sanjay Gupta" and ``\emph{name} Regina Benjamin".
    }
    \label{tab:subtopic}
\end{table*}

==> tables/singletons.tex <==
\begin{table*}[!ht]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{@{}lllllllllllllllllllc@{}}
    \toprule
      \phantom{abcdeffweefbvvefvdsc} & && \multicolumn{3}{c}{MUC} && \multicolumn{3}{c}{$B^3$} && \multicolumn{3}{c}{$CEAFe$} && \multicolumn{3}{c}{LEA} && CoNLL  \\
    
    \cmidrule{4-6} \cmidrule{8-10} \cmidrule{12-14} \cmidrule{16-18} \cmidrule{20-20}
    
    &&& R & P & $F_1$ && R & P & $F_1$ && R &P & $F_1$ && R & P & $F_1$ && $F_1$ \\ 
    
    \midrule 
        \multirow{2}{*}{CoNLL-2012} & S1 && 100 & 60.0 & 75.0 && 100 & 36.1 & 53.1 && 33.3 & 66.7 & 44.4 && 100 & 26.7 & 42.1 && 57.5 \\
        & S2 && 100 & 75.0 & \textbf{85.7} && 100 & 72.2 & \textbf{83.9} && 90.0 & 90.0 & \textbf{90.0} && 100 & 66.7 & \textbf{80.0} && \textbf{86.5} \\
        \midrule
        \multirow{2}{*}{With Singletons} & S1 && 100 & 60.0 & 75.0 && 100 & 63.3 & \textbf{77.6} && 66.7 & 93.3 & \textbf{77.8} && 90.0 & 56.0 & \textbf{69.0} && \textbf{76.8} \\
        & S2 && 100 & 75.0 & \textbf{85.7} && 60.0 & 58.3 & 59.2 && 25.7 & 45.0 & 32.7 && 50.0 & 50.0 & 50.0 && 59.2 \\
    \bottomrule
    \end{tabular}}
    \caption{Coreference results of S1 and S2 when including/omitting singletons.}
    \label{tab:singletons}
\end{table*}

